Voltron: Understanding and Exploiting the Voltage-Latency-Reliability Trade-Offs in Modern DRAM Chips to Improve Energy Efficiency

This paper summarizes our work on experimental characterization and analysis of reduced-voltage operation in modern DRAM chips, which was published in SIGMETRICS 2017, and examines the work's significance and future potential. We take a comprehensive approach to understanding and exploiting the latency and reliability characteristics of modern DRAM when the DRAM supply voltage is lowered below the nominal voltage level specified by DRAM standards. We perform an experimental study of 124 real DDR3L (low-voltage) DRAM chips manufactured recently by three major DRAM vendors. We find that reducing the supply voltage below a certain point introduces bit errors in the data, and we comprehensively characterize the behavior of these errors. We discover that these errors can be avoided by increasing the latency of three major DRAM operations (activation, restoration, and precharge). We perform detailed DRAM circuit simulations to validate and explain our experimental findings. We also characterize the various relationships between reduced supply voltage and error locations, stored data patterns, DRAM temperature, and data retention. Based on our observations, we propose a new DRAM energy reduction mechanism, called Voltron. The key idea of Voltron is to use a performance model to determine by how much we can reduce the supply voltage without introducing errors and without exceeding a user-specified threshold for performance loss. Our evaluations show that Voltron reduces the average DRAM and system energy consumption by 10.5% and 7.3%, respectively, while limiting the average system performance loss to only 1.8%, for a variety of memory-intensive quad-core workloads. We also show that Voltron significantly outperforms prior dynamic voltage and frequency scaling mechanisms for DRAM.

==> sec/subplots/background.tex <==
\begin{figure}[h]
  %\centering
  \captionsetup[subfigure]{justification=centering}

  \subcaptionbox{DRAM System\label{fig:dram-organization}}[0.2\linewidth][l] {
    \vspace{0.6cm}
    \includegraphics[scale=0.65]{plots/background_dram_sys}
}
  \subcaptionbox{DRAM Chip\label{fig:chip-organization}}[0.78\linewidth][r]
  {
    \includegraphics[scale=0.7]{plots/background_dram_chip}
  }%
  \caption{DRAM system and chip organization.}
  \label{fig:background}
\end{figure}


==> sec/subplots/loc_samsung.tex <==
\begin{figure}[!h]
    \centering
    \subcaptionbox{1.05V}[\linewidth]
    {
        \includegraphics{plots/figs/{samsungo13_rcd4_rp4_ret0_temp20_volt1.050000_fix_row}.pdf}
    }

    \subcaptionbox{1.025V}[\linewidth]
    {
        \includegraphics{plots/figs/{samsungo13_rcd4_rp4_ret0_temp20_volt1.025000_fix_row}.pdf}
    }
    \caption{Spatial distribution of errors in a Vendor B's DIMM.}
    \label{fig:locality_B}
\end{figure}


==> sec/subplots/min_latency.tex <==
\begin{figure*}[ht!]
    \centering
    \captionsetup[subfigure]{justification=centering}
    %\subcaptionbox{1}[\linewidth]
    {
        \includegraphics[width=\linewidth]{plots/vendor_bound_tRCD_annotate}
    }

    %\subcaptionbox{2}[\linewidth]
    {
        \includegraphics[width=\linewidth]{plots/vendor_bound_tRP_annotate}
        \vspace{-0.1in}
    }
    \vspace{-0.15in}
    \caption{Distribution of minimum reliable latency values as the supply
      voltage is decreased for 31 DIMMs. The number above each point indicates
      the fraction of DIMMs that \fixIV{work reliably at the specified voltage
      and latency}. Top row: \trcdmin; Bottom row: \trpmin.}
    \label{fig:fpga_latency_range}
\end{figure*}


==> sec/subplots/motivation.tex <==
\begin{figure}[!h]
    \centering
    \captionsetup[subfigure]{justification=centering}
    {
        \includegraphics[width=\linewidth]{plots/powerbreakdown/power_breakdown_Freq_power_isca}
        \vspace{-0.1in}
    }

    {
        \includegraphics[width=\linewidth]{plots/powerbreakdown/power_breakdown_Freq_energy_isca}
        \vspace{-0.1in}
    }

    \caption{Power and energy consumption due to different DRAM frequency.}
    \label{fig:voltron}
\end{figure}


==> sec/subplots/spice_power_energy.tex <==
\begin{figure}[!h]
    \centering
    \captionsetup[subfigure]{justification=centering}[\linewidth]
    {
        \includegraphics[width=\linewidth]{plots/spice_dram_op_energy_over_vdd}
        \vspace{-0.1in}
    }
    \caption{Dynamic energy of DRAM operations as \varr varies.}
    \label{fig:spice_energy_savings}
\end{figure}


==> sec/subplots/target_sweep.tex <==
% -- 4 plots both homo. and hetero. workloads --
%\begin{figure*}[!h]
%    \centering
%    \subcaptionbox*{}[0.49\linewidth][l]
%    {
%      \includegraphics[width=0.47\linewidth]{sim_results/paper_plots/homo_wklds_target_sweep_t1-to-25/voltron_homo_wklds_target_sweep_errorbar_perfloss}
%    }
%    \subcaptionbox*{}[0.49\linewidth][r]
%    {
%      \includegraphics[width=0.47\linewidth]{sim_results/paper_plots/hetero_wklds_target_sweep_t1-to-25/voltron_hetero_wklds_target_sweep_errorbar_perfloss}
%    }
%    \vspace{-0.15in}
%
%    \subcaptionbox{Homogeneous workloads.\label{sweep_homo}}[0.49\linewidth][l]
%    {
%      \includegraphics[width=0.47\linewidth]{sim_results/paper_plots/homo_wklds_target_sweep_t1-to-25/voltron_homo_wklds_target_sweep_errorbar_sysenergysavings}
%    }
%    \subcaptionbox{Heterogeneous workloads.\label{sweep_hetero}}[0.49\linewidth][r]
%    {
%      \includegraphics[width=0.47\linewidth]{sim_results/paper_plots/hetero_wklds_target_sweep_t1-to-25/voltron_hetero_wklds_target_sweep_errorbar_sysenergysavings}
%    }
%    \caption{Performance and energy efficiency of Voltron as the system performance loss target varies.}
%    \label{fig:voltron_sweep}
%\end{figure*}


\begin{figure}[!h]
    \centering
    \subcaptionbox*{}[\linewidth][c]
    {
      \includegraphics[width=\linewidth]{sim_results/paper_plots/hetero_wklds_target_sweep_t1-to-25/voltron_hetero_wklds_target_sweep_errorbar_perfloss}
      \vspace{-0.2in}
    }
    \subcaptionbox*{}[\linewidth][c]
    {
      \includegraphics[width=\linewidth]{sim_results/paper_plots/hetero_wklds_target_sweep_t1-to-25/voltron_hetero_wklds_target_sweep_errorbar_perfwattgains}
    }
    \vspace{-0.2in}
    \caption{System performance loss and energy efficiency improvement of Voltron as the system performance loss target varies.}
    \label{fig:voltron_sweep}
\end{figure}


==> sec/subplots/voltron.tex <==
\begin{figure}[!h]
    \centering
    \captionsetup[subfigure]{justification=centering}
    %\subcaptionbox{1}[\linewidth]
    {
        \includegraphics[width=\linewidth]{plots/voltron_perfloss}
        %\includegraphics[scale=1.0]{plots/voltron_perfloss}
        \vspace{-0.1in}
    }

    %\subcaptionbox{2}[\linewidth]
    {
        \includegraphics[width=\linewidth]{plots/voltron_dramenergysavings}
        %\includegraphics[scale=1.0]{plots/voltron_dramenergysavings}
        \vspace{-0.1in}
    }

    %\subcaptionbox{3}[\linewidth]
    {
        \includegraphics[width=\linewidth]{plots/voltron_sysenergysavings}
        %\includegraphics[scale=1.0]{plots/voltron_sysenergysavings}
        %\vspace{-0.1in}
    }
    \vspace{-0.1in}
    \caption{Comparison between \voltron and an oracle with a system performance
      loss bound of 5\%.}
    \label{fig:voltron}
\end{figure}


==> sec/subplots/voltron_bank_loc.tex <==
\begin{figure}[!h]
    \centering
    \subcaptionbox*{}[0.49\linewidth]
    {
      \includegraphics[width=0.49\linewidth]{sim_results/paper_plots/voltron_bankloc/voltron_voltron_bankloc_ind_box_perfloss}
    }
    %
    \subcaptionbox*{}[0.49\linewidth]
    {
      \includegraphics[width=0.49\linewidth]{sim_results/paper_plots/voltron_bankloc/voltron_voltron_bankloc_ind_box_sysenergysavings}
    }
    \vspace{-0.25in}
    \caption{\fixIV{Performance and energy benefits} of exploiting bank-error locality in Voltron (denoted as
      Voltron+BL) on \fixIV{non-memory-intensive and memory-intensive workloads}.}
    \label{fig:voltron_bankloc}
\end{figure}


==> sec/subplots/voltron_hetero.tex <==
\begin{figure*}[!h]
    \centering
    \subcaptionbox*{}[0.49\linewidth]
    {
      \includegraphics[scale=1.0]{sim_results/paper_plots/hetero_wklds/voltron_hetero_cat_wklds_perfloss}
    }
    %\subcaptionbox*{}[0.33\linewidth]
    %{
    %  \includegraphics[width=0.33\linewidth]{sim_results/paper_plots/hetero_wklds/voltron_hetero_cat_wklds_sysenergysavings}
    %}
    \subcaptionbox*{}[0.49\linewidth]
    {
      \includegraphics[scale=1.0]{sim_results/paper_plots/hetero_wklds/voltron_hetero_cat_wklds_perfwattgains}
    }
    \vspace{-0.25in}

    \caption{\response{System performance loss and energy efficiency improvement of Voltron
        and MemDVFS across 50 different heterogeneous workload mixes.}}
    \label{fig:voltron_hetero}
\end{figure*}


==> sec/subplots/voltron_interval.tex <==
\begin{figure}[!h]
    \centering
    %\captionsetup[subfigure]{justification=left}
    %\subcaptionbox{1}[\linewidth]

    \subcaptionbox*{}[0.49\linewidth][l]
    {
      \includegraphics[scale=1]{sim_results/paper_plots/voltron_homo_intervals/voltron_intervals_drampowersavings}
    }
    \subcaptionbox*{}[0.49\linewidth][r]
    {
      \includegraphics[scale=1]{sim_results/paper_plots/voltron_homo_intervals/voltron_intervals_perfwattgains}
    }
    \vspace{-0.25in}

    \caption{\response{Performance sensitivity of \voltron to profile intervals.}}}
    \label{fig:interval}
\end{figure}


==> sec/subplots/voltron_memdvfs.tex <==
\begin{figure}[!h]
    \centering
    \subcaptionbox{\label{fig:volt_vs_mem_perf}}[0.32\linewidth]
    {
      \includegraphics[scale=1.2]{sim_results/paper_plots/homo_wklds/voltron_homo_wklds_mpki_box_perfloss}
    }
    \subcaptionbox{\label{fig:volt_vs_mem_dpow}}[0.32\linewidth]
    {
      \includegraphics[scale=1.2]{sim_results/paper_plots/homo_wklds/voltron_homo_wklds_mpki_box_drampowersavings}
    }
    \subcaptionbox{\label{fig:volt_vs_mem_syse}}[0.32\linewidth]
    {
      \includegraphics[scale=1.2]{sim_results/paper_plots/homo_wklds/voltron_homo_wklds_mpki_box_sysenergysavings}
    }
    \vspace{-0.15in}
    \caption{\fixIV{Performance and energy} comparison between \voltron and
      \memdvfs on \fixV{non-memory-intensive and memory-intensive workloads}.}
    \label{fig:memdvfs}
\end{figure}


==> sec/subplots/voltron_motivation.tex <==
\begin{figure}[!h]
    \centering
    \captionsetup[subfigure]{justification=centering}
    \subcaptionbox{\fixV{Performance loss vs.\ last-level cache
        MPKI.}\label{fig:mpki}}[\linewidth]
    {
        \includegraphics[width=\linewidth]{plots/linear_regression_motivation_mpki}
    }

    \vspace{0.15in}
    \subcaptionbox{\fixV{Performance loss vs.\ memory stall time fraction.}\label{fig:memstall}}[\linewidth]
    {
        \includegraphics[width=\linewidth]{plots/linear_regression_motivation_stall}
    }
    \vspace{-0.15in}

    \caption{Relationship between performance loss (due to increased
    memory latency) and applications' characteristics: \fixIV{MPKI (a) and memory
    stall time fraction (b)}. Each data point
    represents a single application.}
    \label{fig:voltron_mot}
\end{figure}


==> sec/subplots/vsweep.tex <==
% plots/vsweep_norm_dram_energy.pdf  plots/vsweep_norm_ipc.pdf
% plots/vsweep_norm_system_energy.pdf  plots/vsweep_norm_ws.pdf
\begin{figure*}[t]
    \centering
    \captionsetup[subfigure]{justification=centering}
    {
        \includegraphics[width=\linewidth]{plots/vsweep_norm_ipc}
        \vspace{-0.1in}
    }

    {
        \includegraphics[width=\linewidth]{plots/vsweep_norm_dram_energy}
        \vspace{-0.1in}
    }

    {
        \includegraphics[width=\linewidth]{plots/vsweep_norm_system_energy}
        \vspace{-0.1in}
    }
    \caption{Impact of adjusting DRAM array voltage on system performance and energy
    savings.}
    \label{fig:vsweep}
\end{figure*}


==> sec/subplots/vsweep_high_mpki.tex <==
\begin{figure}[ht]
    \centering
    \captionsetup[subfigure]{justification=centering}
    {
        \includegraphics[width=\linewidth]{plots/vsweep_high_mpki_norm_ipc}
        \vspace{0.1in}
    }

    {
        \includegraphics[width=\linewidth]{plots/vsweep_high_mpki_norm_dram_power}
        \vspace{0.1in}
    }

    {
        \includegraphics[width=\linewidth]{plots/vsweep_high_mpki_norm_system_energy}
        \vspace{-0.1in}
    }
    \caption{System performance loss and energy
    savings due to array voltage scaling for memory-intensive workloads.}
    \label{fig:vsweep_high_mpki}
\end{figure}

